Rethinking Tokenizer and Decoder in Masked Graph Modeling for Molecules

Masked graph modeling excels in the self-supervised representation learning of molecular graphs. Scrutinizing previous studies, we can reveal a common scheme consisting of three key components: (1) graph tokenizer, which breaks a molecular graph into smaller fragments (i.e., subgraphs) and converts them into tokens; (2) graph masking, which corrupts the graph with masks; (3) graph autoencoder, which first applies an encoder on the masked graph to generate the representations, and then employs a decoder on the representations to recover the tokens of the original graph. However, the previous MGM studies focus extensively on graph masking and encoder, while there is limited understanding of tokenizer and decoder. To bridge the gap, we first summarize popular molecule tokenizers at the granularity of node, edge, motif, and Graph Neural Networks (GNNs), and then examine their roles as the MGM's reconstruction targets. Further, we explore the potential of adopting an expressive decoder in MGM. Our results show that a subgraph-level tokenizer and a sufficiently expressive decoder with remask decoding have a large impact on the encoder's representation learning. Finally, we propose a novel MGM method SimSGT, featuring a Simple GNN-based Tokenizer (SGT) and an effective decoding strategy. We empirically validate that our method outperforms the existing molecule self-supervised learning methods. Our codes and checkpoints are available at https://github.com/syr-cn/SimSGT.

==> chapters/1_introduction_v1.tex <==
\section{Introduction}
% Context
% Molecular representation learning is an important topic and have many crucial downstream applications, including drug discovery, retrosynthesis, etc. Because molecules can be represented as graphs, graph self-supervised learning is naturally applied for molecular representation learning. Among all the graph self-supervised learning methods, masked graph modeling has drawn many attention for molecule representation learning. 
Molecular representation learning (MRL)~\cite{MGSSL, Grover} is a critical research area with numerous vital downstream applications, such as molecular property prediction~\cite{GraphCL}, drug discovery~\cite{david2020molecular,MPNN}, and retrosynthesis~\cite{RetroXpert, ucak2022retrosynthetic}. Given that molecules can be represented as graphs, graph self-supervised learning is a natural fit for this problem. Among the various graph self-supervised learning techniques, Masked Graph Modeling (MGM) has recently garnered significant interests~\cite{GraphMAE,molebert,WhenSSL}.

% Context
% In this paper, we study the masked graph modeling for molecule ssl. The goal is to pretrain a graph encoder by denoising a graph autoencoder. The detailed problem formulation:
% •	Graph tokenization: define the reconstruction targets
% •	denoising graph autoencoder
    % o	graph corruption
    % o	graph reconstruction. use a graph network to reconstruct the corrupted tokens
    % o	autoencoder architecture
% The tokenization granularity determines the abstraction level of representations in masked modelling, which is important. Given a token of high-level abstraction (i.e., a motif in graph), it requires an expressive decoder to reconstruct this token for graph denoising. The cooperation between the graph tokenizer and an expressive graph decoder crucially determines the representation quality of MGM.
In this paper, we study MRL through MGM (Figure~\ref{fig:pipeline}), aiming to pretrain a molecule encoder for subsequent fine-tuning in downstream applications. \yuan{By scrutinizing previous works, we summarize that} MGM relies on three key components -- graph tokenizer, graph masking, and graph autoencoder: 
\begin{itemize}[leftmargin=*]
  \item \textbf{Graph tokenizer.} Consider a graph $g$, MGM typically begins by graph tokenization. The graph tokenizer employs a graph fragmentation function~\cite{MGSSL, MoCL, RelMole, Grover} to break $g$ into smaller subgraphs, such as nodes and motifs. Then, these fragments are mapped into fixed-length tokens to serve as the reconstruction targets in MGM. 
  \item \textbf{Graph masking.} MGM then corrupts $g$ by adding random noise, typpically through randomly masking nodes or dropping edges~\cite{pretrain_gnn,WhenSSL}. The corrupted information is later used as self-supervision for pretraining.
  \item \textbf{Graph autoencoder.} Graph autoencoder consists of a graph encoder and a graph decoder. The graph encoder generates the corrupted graph's hidden representations, based on which the graph decoder attempts to recover the corrupted information. The encoder and the decoder are jointly optimized by minimizing the distance between the decoder's outputs and the reconstruction targets, \ie the graph tokens induced by the graph tokenizer. 
  % \yuan{The method of graph fragmentation has been studied in many previous works. However, it remains a open field of exploring them under MGM and applying a more effective mapping function than one-hot encoding.}
\end{itemize}

% 我们有两个贡献, 一个是意识到之前的很多方法做的是 tokenization, 另一个将他们放到 MGM 上测试.

% motivations
% the first motivation
Clearly, the granularity of graph tokens determines the abstraction level of representations in masked modeling~\cite{DALLE, BEiT}. Considering that molecule properties are largely determined by the patterns at the granularity of subgraphs (Figure~\ref{fig:example})~\cite{DBLP:journals/tkde/DeshpandeKWK05}, applying graph tokenizers that generate subgraph-level tokens naturally arises as an idea to improve downstream performances. 
% the second motivation
Further, given the complex subgraph-level tokens as targets, an effective graph reconstruction demands a powerful graph decoder. The cooperation between a subgraph-level graph tokenizer and a powerful graph decoder is vital for learning high-quality molecular representations in MGM.

\begin{figure}[t]
\centering
\begin{minipage}{.5\textwidth}
  \centering
  \includegraphics[width=0.9\linewidth]{figures/pipeline.pdf}
  \caption{The pipeline of Masked Graph Modeling.}
  \label{fig:pipeline}
\end{minipage}%
\hspace{20pt}
\begin{minipage}{.29\textwidth}
  \centering
  \includegraphics[width=\linewidth]{figures/molecule.pdf}
  \caption{Example of subgraph-level patterns in a chemical molecule.}
  \label{fig:example}
\end{minipage}
\end{figure}


% Recovering the token of a node individually falls short in understanding the bigger picture in graphs — how the collaboration of multiple nodes affects the graph properties?


% Review
% The problem of applying graph tokenization in molecular self-supervised learning have been studied in several previous works. (GAP1) Unfortunately, most of these studies are not conducted in the context of MGM~\cite{}.  (Purpose1) We believe a systematic study of existing graph tokenizers in MGM is fundamental. (GAP2) Further, we observe that the importance of applying an expressive graph decoder for subgraph-level tokens have been overlooked. (Purpose2) To resolve the problem, we propose the first MGM method that reconstruct subgraph-level tokens using an expressive graph decoder. Our contributions are two-folds:
% 1) a systematic study of existing tokenizers for molecule self-supervised learning. (details, gnn-based tokenizer, non-parametric tokenizer, other tokenizers, pretrained tokenizers)
% 2) the first framework that uses an expressive graph decoder + subgraph-level token, and achieves the sota performance. (details, two types of decoupling strategy for both GNN and transformer)
\yuan{Previous works have explored motif-based fragmentation functions for MRL~\cite{MGSSL, MoCL, RelMole, Grover}. Unfortunately, these fragmentation functions have been overlooked as tokenizers for MGM.}
% graph tokenizers in molecular self-supervised learning has been explored in several previous studies . Unfortunately, most of these graph tokenizers are not employed as the reconstruction targets in MGM.}
% \yuan{The application of subgraph-level graph tokenizers in molecular self-supervised learning has been explored in several previous studies \cite{MGSSL, MoCL, RelMole, MICRO-Graph, Grover, molebert}. Unfortunately, most of these graph tokenizers are not employed as the reconstruction targets in MGM.} 
We argue that a comprehensive analysis of existing fragmentation functions for their application in MGM's graph tokenization is essential. Moreover, we observe that the significance of employing a powerful graph decoder for reconstructing subgraph-level tokens has been underappreciated. One previous work~\cite{molebert} employs a linear decoder to reconstruct subgraph-level tokens. To address this issue, we introduce the first MGM framework that reconstructs subgraph-level tokens using a powerful graph decoder. Our contributions can be summarized as follows:
\begin{enumerate}[leftmargin=*]
\item We conduct a systematic empirical study of existing graph tokenizers for MRL by MGM. Surprisingly, our findings reveal that a non-parametric Graph Neural Network (GNN) based tokenizer demonstrates competitive or better performance compared to other pretrained and chemistry-inspired tokenizers. Moreover, our analysis shows that reconstructing subgraph-level tokens improves the learning of high-level graph semantics.


% We find the functionalities of encoding and decoding are entangled in the same block of networks in existing graph autoencoders.

% are 
% We find that existing graph autoencoders have entangled encoder and decoder, such that it is not very clear which is which.
\item \yuan{We find that a powerful decoder relieves the encoder's the burden of predicting the corrupted information, and allows the encoder to focus on representation learning, which is more important for downstream performances.} This powerful decoder is achieved by explicitly decoupling the functionalities of the graph encoder and the graph decoder in MGM. \yuan{Without decoupling, the functions of encoding and decoding will be entangled in the same block of networks.} 
Specifically, we present remask \cite{GraphMAE} to decouple GNN-based autoencoders and a variant of remask to decouple Graph Transformer-based~\cite{GraphTrans} autoencoders. Based on the findings above, we introduce the first MGM framework that utilizes a powerful graph decoder to reconstruct subgraph-level tokens.  
\end{enumerate}



% \begin{figure}[t]
%     \centering
% \includegraphics[height=0.2\textwidth]{figures/pipeline}
% % \caption{Example of subgraph-level patterns in a chemical molecule.}
% \label{fig:pipeline}
% % \vspace{-15pt}
% \end{figure}
% \begin{figure}[t]
%     \centering
% \includegraphics[height=0.2\textwidth]{figures/molecule}
% % \caption{Example of subgraph-level patterns in a chemical molecule.}
% \label{fig:example}
% % \vspace{-15pt}
% \end{figure}

% todo: more review on architecture of graph autoencoder

% fixme: need a better review on all MGM frameworks
% fixme: gap1: need talk about the importance of learning high-level semantics? Also, 
% fixme: gap2: need to introduce what is a subgraph-level token?


==> chapters/experiments/4_2_TUDatasets_yrshi.tex <==
\subsection{Unsupervised Learning for Graph Classification}

\textbf{Baselines.} Various state-of-the-art graph pre-training methods with different strategies are compared: node-level grpah reconstruction (GraphMAE \cite{GraphMAE}), graph contrastive learning (GraphCL \cite{GraphCL}, RGCL \cite{RGCL}, AD-GCL \cite{AD-GCL}, JOAO \cite{JOAO}) and mutual information maximization (InfoGraph \cite{InfoGraph}).
% mutual information maximization 的说法可能太过宽泛了，这个有待修改
% this part can be moved before 4.1

\begin{table*}[t]
    \centering
    \caption{Unsupervised learning classification accuracies (\%) on the TU datasets. Performance of other baselines are cited from the original papers. The best results of each column are \textbf{bolded} and the second best results are \underline{underlined}. }
    \label{tab:unsupervised_TU}
    \vspace{6pt}
    \centering\resizebox{1\textwidth}{!}{
        \begin{tabular}{l|cccccccc|cc}\toprule
 Dataset       & NCI1                & PROTEINS            & DD                  & MUTAG               & COLLAB              & RDT-B               & RDT-M5K             & IMDB-B              & AVG            & GAIN \\ \midrule
No Pre-train & 72.67\tiny{±1.16}          & 73.81\tiny{±0.30}          & 77.01\tiny{±0.90}          & 84.26\tiny{±1.16}          & 62.92\tiny{±0.02}          & 72.45\tiny{±0.47}          & 45.32\tiny{±0.30}          & 67.54\tiny{±0.27}          & 69.50         & - \\
InfoGraph    & 78.27±\tiny{0.64}          & 74.56\tiny{±0.57}          & 77.01\tiny{±0.90}          & 87.87\tiny{±1.85}          & 70.73\tiny{±0.48}          & 83.22\tiny{±2.78}          & 55.82\tiny{±0.29}          & 70.96\tiny{±0.60}          & 74.81         & 5.31 \\
GraphCL      & 79.25\tiny{±0.40}    & 74.50\tiny{±0.85}          & 78.24\tiny{±0.99}          & 87.65\tiny{±1.66}          & 71.59\tiny{±0.52}          & \textbf{90.54\tiny{±0.30}} & 55.67\tiny{±0.45}          & 71.38\tiny{±0.40}          & 76.10         & 6.60 \\
JOAO         & 78.57\tiny{±0.17}          & 74.39\tiny{±0.80}          & 77.44\tiny{±0.85}          & 88.85\tiny{±1.51}    & 70.52\tiny{±0.63}          & 88.49\tiny{±0.76}          & \textbf{56.04\tiny{±0.24}} & 71.44\tiny{±0.52}          & 75.72        & 6.22  \\
AD-GCL       & 72.95\tiny{±0.45}          & 73.62\tiny{±0.63}          & 76.06\tiny{±0.44}          & 89.25\tiny{±1.29} & 70.70\tiny{±0.46}          & 87.03\tiny{±1.18}          & 54.81\tiny{±0.42}          & 71.62\tiny{±0.66}          & 74.51         & 5.01 \\
GraphMAE     & 80.29\tiny{±0.23} & 74.91\tiny{±0.58} & 77.88\tiny{±0.69} & 88.84\tiny{±0.99} & 77.98\tiny{±0.68} & 85.48\tiny{±2.65} & 55.14\tiny{±0.26} & \textbf{72.74\tiny{±0.82}} & 76.66 & 7.16\\
R-GCL        & 78.79\tiny{±0.42}          & 74.60\tiny{±0.71}    & \textbf{79.14\tiny{±0.39}} & 88.12\tiny{±1.38}          & 71.44\tiny{±0.60}          & 90.11\tiny{±0.41}    & 55.96\tiny{±0.42}    & 71.84\tiny{±0.76}          & 76.25   & 6.75 \\
SimSGT(Ours)         & \textbf{80.67\tiny{±0.47}} & \textbf{75.00\tiny{±0.11}} & 78.10\tiny{±0.65}          & \textbf{89.91\tiny{±0.66}} & \textbf{79.28\tiny{±0.28}} & 89.31\tiny{±0.56}          & 55.07\tiny{±0.11}          & 72.24\tiny{±1.47} & \textbf{77.45}          & 7.95
            \\\bottomrule
        \end{tabular}
            }
    % \vspace{-13pt}
\end{table*}

We also evaluate SimSGT in the unsupervised representation learning following the setting of \cite{GraphCL}, where graph embeddings generated by unsupervised methods are fed into downstream SVMs for graph-level classification. SimSGT is compared with the above-mentioned graph pre-training schemes on the eight TU datasets, including social networks and biochemical graphs. For each dataset, we perform unsupervised learning on five different random seeds and report the average values along with the standard deviation of accuracies of the five runs. Following \cite{JOAO}, the test accuracy of the epoch with the best validation performance is reported during the test phase. 

In \ref{tab:unsupervised_TU} we represent the unsupervised learning performance on TU datasets. Compared to the state-of-the-art frameworks in \ref{tab:unsupervised_TU}, our method achieves the best average performance among all the datasets and outperforms any other SOTA methods in four out of eight datasets. Using one-hop subgraph representations, our method yields significant performance gains from expressive reconstruction targets, while other graph  methods (e.g., GraphMAE) suffer from a relatively weaker reconstruction task. 

\textbf{Observation 1. Subgraph tokenizer benefits smaller graphs more.} 
It worth noticing that SimSGT achieves the best performance on four out of five datasets with average graph size less than a hundred. For example, on COLLAB, a small social networks dataset with about 74 nodes per sample, our method reaches an accuracy rate of 79.28\%, which is six percentage points ahead of the second-highest method (GraphMAE). On the contrary, contrastive pre-training schemes (GraphCL, JOAO, R-GCL) often have higher accuracies on large graphs. 

% \textbf{Observation 2. Subgraph tokenizer benefits smaller graphs more.} 

\textbf{Hyper-parameter sensitivity.} We also test SimSGT's sensitivity w.r.t. the number of tokenizer layers, number of decoder layers and mask ratio on eight TU datasets under unsupervised learning protocol.
We evaluate our method using different numbers of GIN layers in the tokenizer to prove the effectiveness of a simple subgraph tokenizer. 

\begin{table}[t]
    \centering
    \caption{Unsupervised learning performance on TU datasets with different tokenizer layers. We evaluate our method using different number of GIN layers in tokenizer to prove the effectiveness of . Two-layer GINs are used as decoder in the below experiments.}
    \label{tab:hyperparam-decdepth}
    % \vspace{-6pt}
    \centering\resizebox{0.45\textwidth}{!}{
        \begin{tabular}{l|ccc}
            \toprule
            Decoder depth & 1-layer   & 2-layer    & 3-layer    \\
            \midrule
            Avg. Accuracy(\%)& 77.37\tiny{±0.25} & 77.45\tiny{±0.33} & 76.73\tiny{±0.51}
            \\\bottomrule
        \end{tabular}
            }
    % \vspace{-13pt}
\end{table}

% \begin{table}[t]
%     \centering
%     \caption{Unsupervised learning performance on TU datasets with different tokenizer layers.  Two-layer GINs are used as decoder in the below experiments.}
%     \label{tab:hyperparam-decdepth}
%     % \vspace{-6pt}
%     \centering\resizebox{0.45\textwidth}{!}{
%         \begin{tabular}{l|ccc|c}
%             \toprule
%             Tokenizer depth & DD         & MUTAG      & COLLAB     & AVG        \\
%             \midrule
%             1-layer      & 78.10\tiny{±0.65} & 89.91\tiny{±0.66} & 79.28\tiny{±0.28} & 77.37 \\
%             2-layer      & 78.35\tiny{±0.61} & 87.42\tiny{±1.56} & 77.44\tiny{±0.64} & 77.45 \\
%             3-layer      & 78.88\tiny{±0.17} & 86.91\tiny{±1.13} & 75.76\tiny{±0.75} & 76.73
%             \\\bottomrule
%         \end{tabular}
%             }
%     % \vspace{-13pt}
% \end{table}

\textbf{Observation 3. Social networks may require deeper tokenizers.} 

For small molecule graphs and bioinformatic graphs, the graph-level properties are usually influenced by the existence of dozens of subgraph-level patterns, as known as functional groups or amino acid sequences. In these cases, a single-layer tokenizer which can distinguish hundreds of subgraphs. However for social networks graphs, such kind of subgraph-level patterns are often of unlimited numbers, where a single-layer tokenizer may be not capable for graph reconstruction tasks. In these cases, tokenizers with more GNN layers are repressive might be enough to encode the patterns, but will also introduce additional time cost.

\begin{table}[t]
    \centering
    \caption{Unsupervised learning performance on TU datasets with different decoder layers.}
    \label{tab:hyperparam-tokdepth}
    % \vspace{-6pt}
    \centering\resizebox{0.45\textwidth}{!}{
        \begin{tabular}{l|ccc}
            \toprule
            Tokenizer depth & 1-layer   & 2-layer    & 3-layer    \\
            \midrule
            Avg. Accuracy(\%)& 77.45\tiny{±0.33} & 76.95±0.20 & 76.19±0.23
            \\\bottomrule
        \end{tabular}
            }
    % \vspace{-13pt}
\end{table}

% \begin{table}[t]
%     \centering
%     \caption{Unsupervised learning performance on TU datasets with different decoder layers. Single-layer GINs are used as tokenizer in these experiments. }
%     \label{tab:hyperparam-tokdepth}
%     % \vspace{-6pt}
%     \centering\resizebox{0.45\textwidth}{!}{
%         \begin{tabular}{l|ccc|c}
%             \toprule
%             Decoder depth & DD         & MUTAG      & COLLAB    & AVG \\            
%             \midrule
%             1-layer       & 78.34\tiny{±0.34} & 88.22\tiny{±1.38} & 79.20\tiny{±0.19} & 77.37 \\
%             2-layer       & 78.10\tiny{±0.65} & 89.91\tiny{±0.66} & 79.28\tiny{±0.28} & 77.45 \\
%             3-layer       & 78.01\tiny{±1.10} & 87.13\tiny{±1.89} & 79.06\tiny{±0.39} & 76.73
%             \\\bottomrule
%         \end{tabular}
%             }
%     % \vspace{-13pt}
% \end{table}

% \textbf{Observation 4. The decoder should be neither too deep nor too shallow.} 


\begin{figure}[t]
    \centering
    \includegraphics[width=0.47\textwidth]{chapters/experiments/hyper_mr.pdf}
    \caption{Transfer learning and unsupervised learning performance distributions over different mask ratios.}
    \label{fig:hyperparam-mr}
\end{figure}


\textbf{Ablation Study.} To demonstrate the effectiveness of subgraph-level reconstruction empirically, extensive ablation studies are conducted on TU datasets.


\begin{table}[t]
    \centering
    \caption{Average forward time of 100 batches.}
    \label{tab:speedtest}
    % \vspace{-6pt}
    \begin{tabular}{l|ccc}
        \toprule
        Model type & SGT & MoleBERT    \\
        \midrule
        Forward time (ms) & 0.29 & 2.50
        \\\bottomrule
    \end{tabular}
\end{table}

%  for appendix

\begin{table}[t]
    \centering
    \caption{Hyperparameter used for unsupervised learning}
    \label{tab:hyperparam-unsupervisedTU}
    \centering\resizebox{0.45\textwidth}{!}{
    \begin{tabular}{c|ccccc}
        \toprule
            & learning rate & mask rate & hidden dim & loss type & $\epsilon$ \\
        \midrule
        SimSGT & 0.005         & 0.35      & 32         & sce       & 0.5 \\
        \bottomrule
    \end{tabular}
}
\end{table}
